A Note On Compliance Relations And Fixed Points

We study compliance relations between behavioural contracts in a syntax independent setting based on Labelled Transition Systems. We introduce a fix-point based family of compliance relations, and show that many compliance relations appearing in literature belong to this family.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, A. Mavridou, A. Scalas (Eds.):\\
12th Interaction and Concurrency Experience (ICE 2019).\\
EPTCS 304, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.304.3}{10.4204/EPTCS.304.3}}
\pdfoutput=1

